Simulation of the RIBRAS Facility with GEANT4

A Geant4 simulation code was developed to perform realistic simulations of the RIBRAS facility. A second order expansion of a finite solenoid field was included to describe the beam optics with a good precision. A systematic study of coil currents for several magnetic rigidities and focal points was performed. Parameterizations of the coil currents for single and dual mode operations were obtained. Dedicated routines were developed to simulate the mechanism of direct reactions involving two and three particles in the final state. The present simulations were employed to investigate the feasibility of a Solenoidal Spectrometer with the RIBRAS facility. Our first results indicate that the concept can be applied in the RIBRAS system under certain conditions. Forthcoming studies both from simulations and experiment are already under development.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


